Accelerated Experimental Design for Pairwise Comparisons

Pairwise comparison labels are more informative and less variable than class labels, but generating them poses a challenge: their number grows quadratically in the dataset size. We study a natural experimental design objective, namely, D-optimality, that can be used to identify which $K$ pairwise comparisons to generate. This objective is known to perform well in practice, and is submodular, making the selection approximable via the greedy algorithm. A na\"ive greedy implementation has $O(N^2d^2K)$ complexity, where $N$ is the dataset size, $d$ is the feature space dimension, and $K$ is the number of generated comparisons. We show that, by exploiting the inherent geometry of the dataset--namely, that it consists of pairwise comparisons--the greedy algorithm's complexity can be reduced to $O(N^2(K+d)+N(dK+d^2) +d^2K).$ We apply the same acceleration also to the so-called lazy greedy algorithm. When combined, the above improvements lead to an execution time of less than 1 hour for a dataset with $10^8$ comparisons; the na\"ive greedy algorithm on the same dataset would require more than 10 days to terminate.

==> tex/Author.tex <==
\author{\IEEEauthorblockN{1\textsuperscript{st} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{4\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{6\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
}

==> tex/Experimental_Design.tex <==
As mentioned above, the experimenter augments the dataset by adding comparison labels. It is expensive and time consuming to collect all
$|\mathcal{C}|=\frac{N(N-1)}{2}$ comparison labels. The experimenter thus collects $K$ labels in a subset $\mathcal{S}\subseteq\mathcal{C}$,  $|\mathcal{S}|=K$. In the experimental design problem, we seek a strategy for determining $\mathcal{S}$. To do so, we introduce the objective functions $f:2^{|\mathcal{C}|}\rightarrow \mathbb{R}$, that capture how informative samples in $\mathcal{S}$ are. Given such a function, the optimal subset $\mathcal{S}^{*}$ is a solution to the following problem:
\begin{align}\label{eq:obj}
\begin{split}
\text{Maximize}~~& f(\mathcal{S}),\\
\text{subj.~to}~~&\mathcal{S}\subseteq \mathcal{C}, |\mathcal{S}|=K.
\end{split}
\end{align}
In this paper,our objective is motivated by D-optimal design 
. The D-optimal objective is the negative log entropy of a linear regression model under Gaussian noise. The D-optimal design objective function combined with Bradley-Terry model can be written as:
\begin{align}\label{eq:objective}
f_{D}(\mathcal{S})&=\textstyle\mathop{\log\det}(c I_{d}+\sum_{i\in \mathcal{A}}\bm{x}_{i}\bm{x}_{i}^{T}+\sum_{(i,j)\in \mathcal{S}}\bm{x}_{i,j}\bm{x}_{i,j}^{T})\nonumber\\
&=\mathop{\log\det}(F(\mathcal{A},\mathcal{S})),
\end{align}
where $\bm{x}_{i,j}=\bm{x}_{i}-\bm{x}_{j}$, $c$ is a small positive value, $I_{d}$ is the $d$-dimensional identity matrix, and $\mathcal{A}$ represents the set that has been observed already, $\mathcal{S}$  represents the set should be collected.
$F(\mathcal{A},\mathcal{S})=c I_{d}+\sum_{i\in \mathcal{A}}\bm{x}_{i}\bm{x}_{i}^{T}+\sum_{(i,j)\in \mathcal{S}}\bm{x}_{i,j}\bm{x}_{i,j}^{T}$.




==> tex/Factor_Scalar_Lazy.tex <==
The Naive Lazy approach may not be most efficient which we know from the from the above section. In the lazy iterations, we can also use the factorization tricks. The procedures \textbf{PREPROCESSING}, \textbf{MAXHEAP} and \textbf{FINDMAX} are as same as the Lazy Greedy approach. We just only need some modification for \textbf{UPDATES} and \textbf{UPDATEMARGINAL}. 
\paragraph{UPDATES} Besides what we have done in the same procedure of Lazy Greey, after that we should also do:
\begin{algorithm}[H]
\begin{algorithmic}[1]
\State Decompose matrix $\mathbf{A}^{-1}$ with the form: $\mathbf{A}^{-1}=\mathbf{U}^{T}\mathbf{U}$
\State Calculate and save  $\bm{z}_{i}=\mathbf{U}\bm{x}_{i}$ for all $i\in \mathcal{N}$
\end{algorithmic}
\end{algorithm}

\paragraph{UPDATEMARGINAL} We still need to replace the marginal gain $\Delta(e_{c}|\mathcal{S}_{k})$, but this time by:
\begin{align}
\Delta(e_{c}|\mathcal{S}_{k})\leftarrow ||\bm{z}_{e_{ci}}-\bm{z}_{e_{cj}}||_{2}^{2}
\end{align}


\subsection{Scalar Lazy  Algorithm}
For the Factorization Lazy, for the marginal gain update, we still can't avoid the feature vector inner product.
From the discussion of Scalar Greedy in Sec. \ref{sec:Scalar}, we may use the scalar trick to further decrease the complexity. But for the lazy algorithm, not every item's marginal gain would be updated, so if we want to use the scalar trick we must know when was it last updated. We list the details in the following paragraphs.

\paragraph{PREPROCESSING} It is as same as the previous two algorithms.
\paragraph{MAXHEAP}
In the tuple $h_{e}$, we should also contain the information when it was updated. $h_{e}\leftarrow(d_{e},0, e)$. The other statements are as same as Naive Lazy.
\paragraph{FINDMAX} This step we should extract the item ID $e^{*}$ and $e_{c}$. We should also extract the last updated time $t_{c}$ for item $e_{c}$.  

\begin{algorithm}[H]
\begin{algorithmic}[1]
\State $(\_\_,\_\_,e^{*})\leftarrow\text{Heap-Extract-Max}(\mathbf{H})$ 
\State $(\Delta(e|\mathcal{S}_{t_{c}}),t_{c},e_{c})\leftarrow\mathbf{H}[1]$
\end{algorithmic}
\end{algorithm}

\paragraph{UPDATES}
In this procedure we should save the scalar information between two iterations for every items.

\begin{algorithm}[H]
\begin{algorithmic}[1]
\State Calculate $\bm{v}=\frac{\mathbf{A}^{-1}\bm{x}_{e^{*}}}{\sqrt{1+\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}\bm{x}_{e^{*}}}}$
\State Calculate and save  $\rho_{k,i}=\bm{v}^{T}\bm{x}_{i}$ for all $i\in \mathcal{N}$.

\State $\mathbf{A}^{-1}=\mathbf{A}^{-1}-\bm{v}\bm{v}^{T}$

\State $\mathcal{S}=\mathcal{S}\cup e^{*}$
\end{algorithmic}
\end{algorithm}

\paragraph{UPDATEMARGINAL} For item $e_{c}$ which was last updated at time $t_{c}$, it has the marginal gain $\Delta(e_{c}|\mathcal{S}_{t_{c}})$ in the tuple. Now we can accumulate the differences between iteration $t_{c}$ and $k$ to acquire $\Delta(e_{c}|\mathcal{S}_{k})$.

\begin{algorithm}[H]
\begin{algorithmic}[1]
\State $\Delta(e_{c}|\mathcal{S}_{k})\leftarrow \Delta(e_{c}|\mathcal{S}_{t_{c}})-\underset{t_{c}\leqslant l< k }{\sum}(\rho_{l,e_{ci}}-\rho_{l,e_{cj}})^{2}$
\State $h_{1}\leftarrow(\Delta(e_{c}|\mathcal{S}_{k}),k,e_{c})$
\State $\mathbf{H}[1]\leftarrow h_{1}$
\State Max-Heapify $(\mathbf{H},1)$
\State $(\Delta(e|\mathcal{S}_{t_{c}}),t_{c},opti)\leftarrow\mathbf{H}[1]$.

\end{algorithmic}
\end{algorithm}

\subsection{Memoization Trick}

For the procedure \textbf{UPDATES} in algorithms Factorization Lazy and Scalar Lazy, we calculate all $\bm{z}_{i}$ and $\rho_{k,i}$ for all $i\in\mathcal{N}$. But we know that this may not be indispensable as only part of items may be used. We can use the memoization trick that we calculate $\bm{z}_{i}$ and $\rho_{k,i}$ when it is called the first time in \textbf{UPDATEMARGINAL} procedure. After this, if we use it we can call it directly. We notice that in Python code, this trick may not be fast even in theory it is most saving. The reason may be that the matrix multiplication has been C optimized.




==> tex/Generative_Model.tex <==
We assume that labels are generated according to the following probabilistic model. First, there exists a parameter vector $\bm{\beta}\in\mathbb{R}^{d}$, sampled from a Gaussian prior $\mathcal{N}(0,\sigma^2\bm{I})$, such that for all $i\in\mathcal{N}$ and all $(i,j)\in\mathcal{C}$ the absolute labels $Y_{i}$ and comparison labels $Y_{i,j}$ are independent conditioned on $\bm{\beta}$. Second, the conditional distribution of $Y_{i}$ given $\bm{x}_{i}$ and $\bm{\beta}$ is given by a logistic model, i.e.,
%\begin{subequations}\label{eq:genmod}
\begin{align}\label{eq1}
    \textstyle\mathbf{P}(Y_{i}=+1|\bm{x}_{i},\bm{\beta})=\frac{1}{1+\exp(-\bm{\beta}^{T}\bm{x}_{i})},   \quad i\in \mathcal{N}.
\end{align}
Finally, the conditional distribution of $Y_{i,j}$ given $\bm{x}_{i},\bm{x}_{j}$ and $\bm{\beta}$ is given by the Bradley-Terry model. The Bradley-Terry model assumes that every item $i\in \mathcal{N}$ is associated with a parameter $s_{i}\in \mathbb{R}^{+}$ s.t. 
%\begin{align*}
$\mathbf{P}(Y_{i,j}=+1)=\frac{s_{i}}{(s_{i}+s_{j})}$  for all $(i,j)\in \mathcal{C}.$
%\end{align*} 
We extend this model to incorporate features $\bm{x}_{i}\in\mathbb{R}^{d}, i\in\mathcal{N}$ as follows:
\begin{align}\label{eq2}
    \mathbf{P}(Y_{i,j}\!=\!+1|\bm{x}_{i},\bm{x}_{j},\bm{\beta})=\textstyle\frac{s(\bm{x}_{i},\bm{\beta})}{s(\bm{x}_{i},\bm{\beta})+s(\bm{x}_{j},\bm{\beta})},
    ~(i,j)\in\mathcal{C},
\end{align}

where $s(\bm{x}_{i},\bm{\beta})=\exp(\bm{\beta}^{T}\bm{x}_{i})$. 

%We note that, although the discussion below focuses on a single expert, the probabilistic nature of the model below allows to naturally incorporate  multiple experts, e.g., by having repeated, independent labels over the same comparison pair. 

\begin{table}
\caption{Summary of Notation}\label{tab:notation}
\centering
\normalsize
%\renewcommand{\arraystretch}{1.3}
\begin{tabular}{c|l}
\hline
$N$ & number of items\\
  $i,j$   & comparison item indices \\
    $e$ & candidate index\\
    $e_{i}$ & candidate item's absolute index 
    \\
    $\bm{x}_i$ & absolute feature vector $i$\\
    $\bm{x}_{i,j}$ & $\bm{x}_{i}-\bm{x}_{j}$
    \\
    $\bm{x}_{e}$ &$\bm{x}_{e_{i}}-\bm{x}_{e_{j}}$\\
    $y_i$ & absolute label for $i$\\
    $y_{i,j}$ & comparison outcome between $i$ and $j$ \\
    $s_i$ & Bradley-Terry score for $i$\\
    $\bm{\beta}$ & parameter vector/model in $\mathbb{R}^d$\\
    $\lambda$ & regularization parameter in $\mathbb{R}_+$\\
    $\mathcal{S}$ & collected objective set\\
    $\Delta(e|\mathcal{S})$& marginal gain $f(\mathcal{S}\cup e)-f(\mathcal{S})$\\
    $K$& the final batch size \\
    $k$& the current batch size\\
    $\mathcal{S}_{k}$ & set $\mathcal{S}$ with size $k$ acquired by greedy algorithm\\
    $\Delta(e|\mathcal{S}_{k})$& $f(\mathcal{S}_{k}\cup e)-f(\mathcal{S}_{k})$\\
    \hline
    \end{tabular}
\end{table}

==> tex/Lazy_Part.tex <==
For the D-optimal design, we can see that the fast greedy algorithm still has complexity $O(N^{2}K)$, so we want to use lazy greedy algorithm to optimize the objective function. In this section we discuss how to accelerate the lazy greedy. First we input the same elements such as features and sets like Sec.\ref{sec:aca}. 
\subsection{Lazy Greedy}
\input{tex/LazyGreedy.tex}

\subsection{Naive Lazy Algorithm}
\input{tex/Naive_Lazy.tex}

\subsection{Factorization Lazy Algorithm}
\input{tex/Factor_Scalar_Lazy.tex}

==> tex/Naive_Greedy.tex <==
\begin{lemma}
For a function $f=f_{D}$ in Eq.7,  the Greedy Algorithm is equivalent to the following:
\begin{equation}\label{eq:final objective}
 e^{*}=\underset{e\in \Omega\setminus\mathcal{S}}{\mathbf{argmax}}~~  \bm{x}_{e}\mathbf{A}^{-1}\bm{x}_{e}    
\end{equation}
\end{lemma}

\begin{proof}
Now for each iteration step,  the matrix $\mathbf{A}_{k}$ is a positive definite matrix. Using the matrix determinant lemma, we have the following:

Now based on the matrix determinant lemma, we know that:
\begin{align}
\begin{split}
    e^{*}&=\underset{e\in \Omega\setminus\mathcal{S}}{\mathbf{argmax}}\mathop{det}(\mathbf{A})(1+\bm{x}_{e}^{T}\mathbf{A}^{-1}\bm{x}_{e})
    \\&=\underset{e\in \Omega\setminus\mathcal{S}}{\mathbf{argmax}}~~  \bm{x}_{e}\mathbf{A}^{-1}\bm{x}_{e}
\end{split}
\end{align}
\end{proof}



%We can notice from step $k$ to step $k+1$, besides adding element to the set $\mathcal{S}$, the matrix $\mathbf{A}_{k}$ should also be updated. We should use the Sherman-Morrison formular.


%We can summarize the above discussions and form the Naive Algorithm:





==> tex/Naive_Lazy.tex <==
As we discussed in Sec. \ref{subsec:naive}, we can redefine the $d_{e}=\bm{x}_{e}\mathbf{A}^{-1}\bm{x}_{e}$, we can use it as the marginal gain in the Alg.\ref{alg:lazygreedy} for simplicity.
\paragraph{PREPROCESSING}
To build up the max heap, we should prepare $d_{e}$ for each item $e\in \Omega$.  We know the factorization can decease the complexity of preparation from Sec.\ref{sec:fga}, and Sec.\ref{sec:Scalar}. We should prepare $d_{e}$ with factorization trick:
\begin{algorithm}[H]
\begin{algorithmic}[1]
\State Calculate the inverse $\mathbf{A}^{-1}$.
\State Calculate $\mathbf{U}$: decompose the matrix $\mathbf{A}^{-1}$ into $\mathbf{U}^{T}\mathbf{U}$ by Cholesky decomposition.
	
\State Calculate and save  $\bm{z}_{i}=\mathbf{U}\bm{x}_{i}$ for all $i\in \mathcal{N}$. 
\State Calculate and save $d_{e}=||\bm{z}_{e_{i}}-\bm{z}_{e_{j}}||_{2}^{2}$ for all $e\in \Omega\setminus\mathcal{S}$.
\end{algorithmic}
\end{algorithm}
For the other algorithms in this section, we will also do the same preprocessing procedure as this part.

\paragraph{MAXHEAP} For this process, we only replace marginal gain $\Delta(e|\mathcal{S}_{0})$ by $d_{e}$, $h_{e}\leftarrow(d_{e},0, e)$.

\paragraph{FINDMAX} This procedure will be same as Alg.\ref{alg:lazygreedy}.

\paragraph{UPDATES} Besides the statements in Alg.\ref{alg:lazygreedy}, we should also renew the inverse of $\mathbf{A}$ by Eq.\ref{eq:adapt}.

\paragraph{UPDATEMARGINAL} For the marginal gain update, we should also avoid using marginal gain $\Delta(e_{c}|\mathcal{S}_{k})$ directly, but use $\bm{x}_{e_c}\mathbf{A}^{-1}\bm{x}_{e_c}$ instead.


	



==> tex/Posteriori_Estimation.tex <==
After the collection of comparison labels, the  dataset available to the experimenter consists of absolute labels
in subset $\mathcal{A}\subseteq\mathcal{N}$ and comparison labels in subset $\mathcal{S}\subseteq\mathcal{C}$. The experimenter can train a classifier through maximum a posteriori estimation (MAP) over the generative model presented in Sec. \ref{sec:gm}. Then, the estimation of  parameter vector $\bm{\beta}$ amounts to minimizing the following negative log-likelihood function:
\begin{equation}\label{eq4}
\begin{split}
\mathcal{L}(\bm{\beta};\mathcal{A},\mathcal{S}) =&\textstyle \sum_{i\in \mathcal{A}}\mathbf{log}(1+e^{-y_i\bm{\beta}^T\bm{x_i}})
\\
\textstyle+\sum_{(i,j)\in \mathcal{S}}&\mathbf{log}(1+e^{-y_{i,j}\bm{\beta}^T(\bm{x_i}-\bm{x_j})})+\lambda ||\bm{\beta}||_{2}^{2},
\end{split}
\end{equation}
where the penalty coefficient $\lambda$ equals $1/\sigma^{2}$, and in practice is determined  through cross-validation. 


==> tex/bibcite.tex <==
\bibitem{sculley2010combined}
D, Sculley. { Combined regression and ranking.} In SIGKDD, 2010.

\bibitem{kalpathy2016plus}
J. Kalpathy-Cramer, J. P. Campbell, D. Erdogmus, P. Tian, D. Kedarisetti, C. Moleta, J. D. Reynolds et al. {\em Plus disease in retinopathy of prematurity: improving diagnosis by ranking disease severity and using quantitative image analysis.}  Ophthalmology 123, no. 11, 2016


\bibitem{desarkar2010aggregating}
M. S. Desarkar, S. Sarkar, and P. Mitra. {\em Aggregating preference graphs for collaborative rating prediction.} In Recsys, pp.21-28, 2010.

\bibitem{desarkar2012preference}
  M. S. Desarkar, R. Saxena, and S. Sarkar. {\em Preference relation based matrix factorization for recommender systems} In UMAP, pp. 63-75. Springer, 2012.

\bibitem{guo}
 Y. Guo, P. Tian, J. Kalpathy-Cramer, S. Ostmo, J. P. Campbell, M. F. Chiang, D. Erdogmus, J. G. Dy, and S. Ioannidis. {\em Experimental Design under the Bradley-Terry Model.} In IJCAI, pp. 2198-2204, 2018.

\bibitem{stewart2005absolute}
N. Stewart, G. DA Brown, and N. Chater. {\em Absolute identification by relative judgment.} Psychological review 112, p.881 , 2005.

\bibitem{brun2010towards}
 A. Brun, A. Hamad, O. Buffet, and A. Boyer. {\em Towards preference relations in recommender systems.} In  ECML/PKDD Workshop, 2010.

\bibitem{zheng2009mining}
Y. Zheng, L. Zhang, X. Xie, and W.Y. Ma. {\em Mining interesting locations and travel sequences from GPS trajectories.} In WWW, pp. 791-800. ACM, 2009.

\bibitem{koren2011ordrec}
Y. Koren,  and J. Sill. {\em OrdRec: an ordinal model for predicting personalized item rating distributions.} In Recsys, pp. 117-124. ACM, 2011.

\bibitem{schultz2004learning}
M. Schultz,  and T. Joachims. {\em Learning a distance metric from relative comparisons.} In NIPS, pp. 41-48. 2004.

\bibitem{boyd2004convex}
 S. Boyd, and L. Vandenberghe. {\em Convex optimization.} Cambridge university press, 2004.
 
\bibitem{pukelsheim1993optimal}
 F. Pukelsheim,{\em Optimal design of experiments.} Vol. 50. SIAM, 1993.
 
\bibitem{nemhauser1978}
 G. L. Nemhauser, L. A. Wolsey, and M. L. Fisher. {\em An analysis of approximations for maximizing submodular set functions—I.} Mathematical programming pp.265-294, 1978
 
 \bibitem{van1996matrix}
 G. H. Golub, and C. F. Van Loan. {\em Matrix computations.} Vol. 3. JHU Press, 2012.    
 \bibitem{sherman1950adjustment}
  J. Sherman, and W. J. Morrison. {\em Adjustment of an inverse matrix corresponding to a change in one element of a given matrix.} The Annals of Mathematical Statistics pp. 124-127. 1950
\bibitem{minoux1978accelerated}
 M. Minoux, {\em Accelerated greedy algorithms for maximizing submodular set functions.} In Optimization techniques, pp. 234-243. Springer, 1978.
 \bibitem{mirzasoleiman2015lazier}
  B. Mirzasoleiman, A. Badanidiyuru, A. Karbasi, J. Vondrák, and A. Krause. {\em Lazier Than Lazy Greedy.} In AAAI, pp. 1812-1818. 2015.
\bibitem{lin2011class}  
 H.Lin, and J. Bilmes. {\em A class of submodular functions for document summarization.} In HLT, pp. 510-520, 2011.
\bibitem{mirzasoleiman2013distributed} 
B. Mirzasoleiman, A. Karbasi, R. Sarkar, and A. Krause. {\em Distributed submodular maximization: Identifying representative elements in massive data.} In NIPS pp. 2049-2057. 2013.
 
\bibitem{chen2015fusing}
  L.Chen, P. Zhang, and B. Li. {\em Fusing pointwise and pairwise labels for supporting user-adaptive image retrieval.} In ICMR, pp. 67-74. ACM, 2015.
 \bibitem{takamura2015estimating}
 H. Takamura, and Jun'ichi Tsujii. {\em Estimating numerical attributes by bringing together fragmentary clues.} In HLT, pp. 1305-1310, 2015.
 \bibitem{wang2016ppp}
  Y.Wang, S. Wang, J. Tang, H. Liu, and B. Li. {\em Ppp: Joint pointwise and pairwise image label prediction.} In CVPR, pp. 6005-6013， 2016.
 \bibitem{active}
  K. G. Jamieson, and N. Robert. {\em Active ranking using pairwise comparisons." In Advances in Neural Information Processing Systems.} pp. 2240-2248. 2011.
 
 %\bibitem{ryan2003estimating}
 %K.J. Ryan, {\em Estimating expected information gains for experimental designs with application to the random fatigue-limit model.} Journal of Computational and Graphical Statistics 12, pp.585-603, 2003. 
 \bibitem{liepe2013maximizing}
 J. Liepe, S. Filippi, M. Komorowski, and M. PH. Stumpf. {\em Maximizing the information content of experiments in systems biology.} PLoS computational biology 9, e1002888. 2013.
 
 \bibitem{cavagnaro2010adaptive}
 D. R. Cavagnaro, J. I. Myung, M. A. Pitt, and J. V. Kujala. {\em Adaptive design optimization: A mutual information-based approach to model discrimination in cognitive science.} Neural computation pp. 887-905, 2010.
 
 \bibitem{krause2012near}
 A. Krause, and C. E. Guestrin. {\em Near-optimal nonmyopic value of information in graphical models.} arXiv preprint arXiv:1207.1394, 2012
 
\bibitem{busetto2013near}
 A. G. Busetto, A. Hauser, G. Krummenacher, M. Sunnåker, S. Dimopoulos, C. S. Ong, J. Stelling, and J. M. Buhmann. {\em Near-optimal experimental design for model selection in systems biology.} Bioinformatics  pp.2625-2632, 2013.

\bibitem{krause2014submodular}
 A. Krause, and D. Golovin. {\em Submodular function maximization.} pp. 71-104. 2014
 \bibitem{golovin2011adaptive}
 D. Golovin, and A. Krause. {\em Adaptive submodularity: Theory and applications in active learning and stochastic optimization.} In JAIR, 42, pp. 427-486, 2011
 
% \bibitem{grasshoff2003optimal}
 %U. Grasshoff*, H. Großmann, H. Holling, and R. Schwabe. {\em Optimal paired comparison designs for first-order interactions.} Statistics pp. 373-386, 2003

\bibitem{glickman2005adaptive}
 M. E. Glickman, and S. T. Jensen. {\em Adaptive paired comparison design.} Journal of statistical planning and inference, pp.279-293, 2005
 
\bibitem{leskovec2007cost}
 J. Leskovec, A. Krause, C. Guestrin, C. Faloutsos, J. VanBriesen, and N. Glance. {\em Cost-effective outbreak detection in networks.} In SIGKDD, pp. 420-429, 2007.
 
\bibitem{gomez2012inferring}
 M. Gomez-Rodriguez, J. Leskovec, and A. Krause. {\em Inferring networks of diffusion and influence.} in TKDD, p.21, 2012
\bibitem{xiao2013lazy}
 H. Xiao, and C. Eckert. {\em Lazy Gaussian Process Committee for Real-Time Online Regression.} In AAAI. 2013
\bibitem{wei2015submodularity}
 K. Wei, R. Iyer, and J. Bilmes. {\em Submodularity in data subset selection and active learning.} In ICML, pp.1954-1963, 2015.
 
 \bibitem{bradley1952rank}
 R. A. Bradley, and M. E. Terry. {\em Rank analysis of incomplete block designs: I. The method of paired comparisons.} Biometrika pp.324-345, 1952
 
\bibitem{he2010laplacian}
 X. He, {\em Laplacian regularized D-optimal design for active learning and its application to image retrieval.} IEEE Transactions on Image Processing. pp. 254-263, 2010
 
 %\bibitem{chaloner1989optimal}
% K. Chaloner, and K. Larntz. {\em Optimal Bayesian design applied to logistic regression experiments.} Journal of statistical planning and inference pp. 191-208, 1989.
 
\bibitem{grasshoff2008optimal}
U. Graßhoff, and R. Schwabe. {\em Optimal design for the Bradley–Terry paired comparison model.} Statistical Methods and Applications pp. 275-289, 2008

\bibitem{harville1997matrix}
 D. A. Harville, {\em Matrix algebra from a statistician's perspective.} Springer, 1997.
 
\bibitem{press2007numerical} W. H. Press, S. A. Teukolsky, W. T. Vetterling, and B. P. Flannery. {\em Numerical recipes 3rd edition: The art of scientific computing.} Cambridge university press, 2007.

\bibitem{hager1989updating}
 W. W. Hager, {\em Updating the inverse of a matrix.} SIAM review pp. 221-239. 1989

%\bibitem{coppersmith1987matrix}
% D. Coppersmith, and S. Winograd. {\em Matrix multiplication via arithmetic progressions.} In STOC, pp. 1-6. ACM, 1987.

\bibitem{krause2007near}
A. Krause,  and C. Guestrin. {\em Near-optimal observation selection using submodular functions.} In AAAI, pp.1650-1654. 2007.

\bibitem{changshui2011fast}
C, Zhang,  G. Hou, and J. Wang  {\em A fast algorithm based on the submodular property for optimization of wind turbine positioning.} Renewable Energy 36, pp. 2951-2958. 2011

\bibitem{liu2011entropy}
 Ming-Yu Liu, O. Tuzel, S. Ramalingam, and R. Chellappa. {\em Entropy rate superpixel segmentation.} In CVPR, pp. 2097-2104. 2011.
\bibitem{calinescu2011maximizing}
 G. Calinescu, C. Chekuri, M. Pál, and J. Vondrák. {\em Maximizing a monotone submodular function subject to a matroid constraint.} SIAM Journal on Computing 40, pp. 1740-1766. 2011
\bibitem{krause2008near}
A. Krause,  A. Singh, and C. Guestrin. {\em Near-optimal sensor placements in Gaussian processes: Theory, efficient algorithms and empirical studies.} Journal of Machine Learning Research pp. 235-284. 2008

\bibitem{sun2015submodboxes}
Q. Sun, and D. Batra. {\em Submodboxes: Near-optimal search for a set of diverse object proposals.} In NIPS, pp. 1378-1386. 2015.

\bibitem{brown2018fully}
J. M. Brown,  J. Peter Campbell, A. Beers, K. Chang, K. Donohue, S. Ostmo, RV Paul Chan et al. {\em Fully automated disease severity assessment and treatment monitoring in retinopathy of prematurity using deep learning.} In Medical Imaging, 2018

\bibitem{kamishima2009trbagg}
 T. Kamishima, M. Hamasaki, and S. Akaho. {\em TrBagg: A simple transfer learning method and its application to personalization in collaborative tagging.} In ICDM, pp. 219-228. IEEE, 2009.

\bibitem{elo1978rating}
A. E. Elo,  {\em The rating of chessplayers, past and present} Arco Pub., 1978.

\bibitem{koren2009matrix}
 Y. Koren, R. Bell, and C. Volinsky. {Matrix factorization techniques for recommender systems.} Computer 8: pp. 30-37. 2009

%\bibitem{maystre2015just}
% L. Maystre, and M. Grossglauser. {\em  Just Sort It! A Simple and Effective Approach to Active Preference Learning.} In ICML, pp. 2344-2353. 2017.
 
\bibitem{DBLP:journals/corr/QinL13}
T. Qin, and Tie-Yan Liu. {\em Introducing LETOR 4.0 datasets.} arXiv preprint arXiv:1306.2597. 2013.

\bibitem{Dua:2017}
D. Dheeru, and E. K. Taniskidou. {\em UCI machine learning repository.} University of California, Irvine, School of Information and Computer Sciences. 2017.


\bibitem{bento2011identifying}
J. Bento, N. Fawaz, A. Montanari, and S. Ioannidis. {\em Identifying users from their rating patterns.} In CAMRa, pp. 39-46. ACM, 2011.

==> tex/pseudocode.tex <==
\begin{algorithm}[H]
\caption{Scalar Lazy Greedy}\label{heap}
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $\mathbf{A}\in \mathbb{S}_{+}^{d}, \bm{x}_{1},\bm{x}_{2},\cdots,\bm{x}_{N}\in\mathbb{R}^{d}, \Omega=\{(i,j):  i,j\in \mathcal{N}, i<j\}, |\Omega|=\omega.$
    
    \State Decompose matrix $\mathbf{A}^{-1}$ with the form: $\mathbf{A}^{-1}=\mathbf{U}^{T}\mathbf{U}$
    
	\State Calculate and save  $\bm{z}_{i}=\mathbf{U}\bm{x}_{i}$ for all $i\in \mathcal{N}$ 
	\State Build up  tuples for all   $(\Delta(e|\mathcal{S}_{0})=||\bm{z}_{e_{i}}-\bm{z}_{e_{j}}||_{2}^{2},0,e)$ for all $e\in \Omega$.
	\State $\mathbf{H}=[(\Delta(e_{1}|\mathbf{S}_{0}),0,e_{1}),\cdots,(\Delta(e_{\omega}|\mathbf{S}_{0}),0,e_{\omega})].$
    \State\textbf{MaxHeapify}$(\mathbf{H})$.
    \State $k=0$.
	\While{$\mathbf{True}$:}
	\State $(\_\_,\_\_,e^{*})=$heappop($\mathbf{H}$).
    \State$\mathcal{S}=\mathcal{S}\cup e^{*}$
    
    \If{$|\mathcal{S}|\geqslant K$}
    \State \textbf{break}.
    \EndIf
    
    \State Calculate $\bm{v}_{k}=\frac{\mathbf{A}^{-1}\bm{x}_{e^{*}}}{\sqrt{1+\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}\bm{x}_{e^{*}}}}$
	\State Calculate and save  $\rho_{k,i}=\bm{v}_{k}^{T}\bm{x}_{i}$ for all $i\in \mathcal{N}$.
	
	\State $k+=1$
    \State $\mathbf{A}^{-1}=\mathbf{A}^{-1}-\frac{\mathbf{A}^{-1}\bm{x}_{e^{*}}\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}}{1+\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}\bm{x}_{e^{*}}}$
    
	\State $(\Delta(e_{c}|\mathcal{S}_{t}),t,e_{c})\leftarrow \mathbf{H}[1]$.
	\While{$\mathbf{True}$:}
	\State $\Delta(e_{c}|\mathcal{S}_{k})\leftarrow \Delta(e_{c}|\mathcal{S}_{t})-\underset{t\leqslant l< k }{\sum}(\rho_{l,e_{ci}}-\rho_{l,e_{cj}})^{2}$
	\State heapreplace$(\mathbf{H}, (\Delta(e_{c}|\mathcal{S}_{k}),k,e_{c}) )$
	\State $(\Delta(e_{c}|\mathcal{S}_{t}),t,opti)\leftarrow \mathbf{H}[1]$.
	
	\If{$opti==e_{c}$}
	\State \textbf{break}.
	\Else
	\State $e_{c}=opti$
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\caption{Factorization Lazy Greedy}\label{heap}
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $\mathbf{A}\in \mathbb{S}_{+}^{d}, \bm{x}_{1},\bm{x}_{2},\cdots,\bm{x}_{N}\in\mathbb{R}^{d}, \Omega=\{(i,j):  i,j\in \mathcal{N}, i<j\}, |\Omega|=\omega.$
    
    \State Decompose matrix $\mathbf{A}^{-1}$ with the form: $\mathbf{A}^{-1}=\mathbf{U}^{T}\mathbf{U}$
    
	\State Calculate and save  $\bm{z}_{i}=\mathbf{U}\bm{x}_{i}$ for all $i\in \mathcal{N}$ 
	\State Build up  tuples for all   $(\Delta(e|\mathcal{S}_{0})=||\bm{z}_{e_{i}}-\bm{z}_{e_{j}}||_{2}^{2},e)$ for all $e\in \Omega$.
	\State $\mathbf{H}=[(\Delta(e_{1}|\mathbf{S}_{0}),e_{1}),(\Delta(e_{2}|\mathbf{S}_{0}),e_{2}),\cdots,(\Delta(e_{\omega}|\mathbf{S}_{0}),e_{\omega})].$
    \State\textbf{MaxHeapify}$(\mathbf{H})$. 
	\While{$\mathbf{True}$:}
	\State $(\_\_,e^{*})=$heappop($\mathbf{H}$).
    \State$\mathcal{S}=\mathcal{S}\cup e^{*}$
    \If{$|\mathcal{S}|\geqslant K$}
    \State \textbf{break}
    \EndIf
    \State $\mathbf{A}^{-1}=\mathbf{A}^{-1}-\frac{\mathbf{A}^{-1}\bm{x}_{e^{*}}\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}}{1+\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}\bm{x}_{e^{*}}}$
    \State Decompose matrix $\mathbf{A}^{-1}$ with the form: $\mathbf{A}^{-1}=\mathbf{U}^{T}\mathbf{U}$
	\State Calculate and save  $\bm{z}_{i}=\mathbf{U}\bm{x}_{i}$ for all $i\in \mathcal{N}$
	
	\State $(\_\_,e_{c})\leftarrow \mathbf{H}[1]$ .
	\While{$\mathbf{True}$:}
	\State $\Delta(e_{c}|\mathcal{S}_{k})\leftarrow ||\bm{z}_{e_{ci}}-\bm{z}_{e_{cj}}||_{2}^{2}$
	\State heapreplace$(\mathbf{H}, (\Delta(e_{c}|\mathcal{S}_{k}),e_{c}) )$
	\State $(\_\_,opti)\leftarrow \mathbf{H}[1]$.
	
	\If{$opti==e_{c}$}
	\State \textbf{break}.
	\Else
	\State $e_{c}=opti$
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\caption{Naive Lazy Greedy}\label{heap}
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $\mathbf{A}\in \mathbb{S}_{+}^{d}, \bm{x}_{1},\bm{x}_{2},\cdots,\bm{x}_{N}\in\mathbb{R}^{d}, \Omega=\{(i,j):  i,j\in \mathcal{N}, i<j\},|\Omega|=\omega$.
	\State Build up  tuples    $(\Delta(e|\mathcal{S}_{0})=\bm{x}_{e}^{T}\mathbf{A}^{-1}\bm{x}_{e}, e)$ for all $e\in \Omega$.
	\State $\mathbf{H}=[(\Delta(e_{1}|\mathbf{S}_{0}),e_{1}),(\Delta(e_{2}|\mathbf{S}_{0}),e_{2}),\cdots,(\Delta(e_{\omega}|\mathbf{S}_{0}),e_{\omega})].$
    \State\textbf{MaxHeapify}$(\mathbf{H})$. 
	\While{$\mathbf{True}$:}
	\State $(\_\_,e^{*})=$heappop($\mathbf{H}$).
    \State$\mathcal{S}=\mathcal{S}\cup e^{*}$
    \If{$|\mathcal{S}|\geqslant K$}
    \State \textbf{break}
    \EndIf
    \State $\mathbf{A}^{-1}=\mathbf{A}^{-1}-\frac{\mathbf{A}^{-1}\bm{x}_{e^{*}}\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}}{1+\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}\bm{x}_{e^{*}}}$
	\State $(\_\_,e_{c})\leftarrow \mathbf{H}[1]$ .
	\While{$\mathbf{True}$:}
	\State \textbf{UPDATEMARGINAL} %$\Delta(e_{c}|\mathcal{S}_{k})\leftarrow \bm{x}_{e_{c}}^{T}\mathbf{A}^{-1}\bm{x}_{e_{c}}$
	%\State heapreplace$(\mathbf{H}, (\Delta(e_{c}|\mathcal{S}_{k}),e_{c}) )$
	%\State $(\_\_,opti)\leftarrow \mathbf{H}[1]$.
	
	\If{$opti==e_{c}$}
	\State \textbf{break}.
	\Else
	\State $e_{c}=opti$
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}

==> tex/save.tex <==
\begin{algorithm}[H]
\caption{LazyGreedy}\label{heap}
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $f, \Omega$,$|\Omega|=\omega$
	\State Build up  tuples   $(\Delta(e|\mathcal{S}_{0})=f(e)-f(\emptyset), e)$ for all $e\in \Omega$.
	\State $\mathbf{H}=[(\Delta(e_{1}|\mathbf{S}_{0}),e_{1}),(\Delta(e_{2}|\mathbf{S}_{0}),e_{2}),\cdots,(\Delta(e_{\omega}|\mathbf{S}_{0}),e_{\omega})].$
    \State\textbf{MaxHeapify}$(\mathbf{H})$. 
	\While{$\mathbf{True}$:}
	\State $(\_\_,e^{*})=$heappop($\mathbf{H}$).
    \State$\mathcal{S}=\mathcal{S}\cup e^{*}$
    \If{$|\mathcal{S}|\geqslant K$}
    \State \textbf{break}
    \EndIf
	\State $(\_\_,e_{c})\leftarrow \mathbf{H}[1]$ .
	\While{$\mathbf{True}$:}
	\State $\Delta(e_{c}|\mathcal{S}_{k})\leftarrow f(\mathcal{S}_{k}\cup e_{c})-f(\mathcal{S}_{k})$
	\State heapreplace$(\mathbf{H}, (\Delta(e_{c}|\mathcal{S}_{k}),e_{c}) )$
	\State $(\_\_,opti)\leftarrow \mathbf{H}[1]$.
	
	\If{$opti==e_{c}$}
	\State $\textbf{break}$.
	\Else
	\State $e_{c}=opti$
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm} 

\begin{algorithm}[H]
\caption{Factorization Lazy Greedy}\label{heap}
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $\mathbf{A}\in \mathbb{S}_{+}^{d}, \bm{x}_{1},\bm{x}_{2},\cdots,\bm{x}_{N}\in\mathbb{R}^{d}, \Omega=\{(i,j):  i,j\in \mathcal{N}, i<j\}, |\Omega|=\omega.$
    
    \State Decompose matrix $\mathbf{A}^{-1}$ with the form: $\mathbf{A}^{-1}=\mathbf{U}^{T}\mathbf{U}$
    
	\State Calculate and save  $\bm{z}_{i}=\mathbf{U}\bm{x}_{i}$ for all $i\in \mathcal{N}$ 
	\State Build up  tuples for all   $(\Delta(e|\mathcal{S}_{0})=||\bm{z}_{e_{i}}-\bm{z}_{e_{j}}||_{2}^{2},e)$ for all $e\in \Omega$.
	\State $\mathbf{H}=[(\Delta(e_{1}|\mathbf{S}_{0}),e_{1}),(\Delta(e_{2}|\mathbf{S}_{0}),e_{2}),\cdots,(\Delta(e_{\omega}|\mathbf{S}_{0}),e_{\omega})].$
    \State\textbf{MaxHeapify}$(\mathbf{H})$. 
	\While{$\mathbf{True}$:}
	\State $(\_\_,e^{*})=$heappop($\mathbf{H}$).
    \State$\mathcal{S}=\mathcal{S}\cup e^{*}$
    \If{$|\mathcal{S}|\geqslant K$}
    \State \textbf{break}
    \EndIf
    \State $\mathbf{A}^{-1}=\mathbf{A}^{-1}-\frac{\mathbf{A}^{-1}\bm{x}_{e^{*}}\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}}{1+\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}\bm{x}_{e^{*}}}$
    \State Decompose matrix $\mathbf{A}^{-1}$ with the form: $\mathbf{A}^{-1}=\mathbf{U}^{T}\mathbf{U}$
	\State Calculate and save  $\bm{z}_{i}=\mathbf{U}\bm{x}_{i}$ for all $i\in \mathcal{N}$
	
	\State $(\_\_,e_{c})\leftarrow \mathbf{H}[1]$ .
	\While{$\mathbf{True}$:}
	\State $\Delta(e_{c}|\mathcal{S}_{k})\leftarrow ||\bm{z}_{e_{ci}}-\bm{z}_{e_{cj}}||_{2}^{2}$
	\State heapreplace$(\mathbf{H}, (\Delta(e_{c}|\mathcal{S}_{k}),e_{c}) )$
	\State $(\_\_,opti)\leftarrow \mathbf{H}[1]$.
	
	\If{$opti==e_{c}$}
	\State \textbf{break}.
	\Else
	\State $e_{c}=opti$
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}

\begin{figure}[H]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.6\columnwidth,height=0.6\columnwidth]{pic/aucplot2.pdf}}
\begin{small}
\caption{Average AUC for the synthetic data with feature dimension $d=30$.}
\end{small}
\label{fig:GM}
\end{center}
\vskip -0.2in
\end{figure}

\begin{figure}[H]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.6\columnwidth,height=0.6\columnwidth]{pic/aucplot3.pdf}}
\begin{small}
\caption{Average AUC for the synthetic data with feature dimension $d=100$ .}
\end{small}
\label{fig:GM}
\end{center}
\vskip -0.2in
\end{figure}


\begin{comment}
\begin{table}[h]
\centering
\caption{The Data Information}
\label{graspPercentage}
\footnotesize
\begin{tabular}[b]{ccccc}
\toprule
\bf{Dataset} & \bf{N} & \bf{d}&$|\mathcal{C}|$ &$|\mathcal{A}|$\\
\midrule
SynData & 3000 & 20\\
ROP & 100 & 156\\

\midrule
\end{tabular}
\end{table}
\end{comment}

\begin{algorithm}[H]
\label{alg:greedy}
\caption{Greedy Algorithm} 
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
	\While{$|\mathcal{S}| \leqslant K$}\State
	$\bm{e^{*}}=\underset{(i,j)\in \mathcal{C}\setminus\mathcal{S}}{\mathbf{argmax}}f(\mathcal{S}\cup \{(i,j)\})-f(\mathcal{S})$	\State $\mathcal{S}=\mathcal{S} \cup e^{*} $
	\EndWhile
	\State \Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
\caption{Naive Lazy Greedy}\label{heap}
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $\mathbf{A}\in \mathbb{S}_{+}^{d}, \bm{x}_{1},\bm{x}_{2},\cdots,\bm{x}_{N}\in\mathbb{R}^{d}, \Omega=\{(i,j):  i,j\in \mathcal{N}, i<j\},|\Omega|=\omega$.
	\State Build up  tuples    $(\Delta(e|\mathcal{S}_{0})=\bm{x}_{e}^{T}\mathbf{A}^{-1}\bm{x}_{e}, e)$ for all $e\in \Omega$.
	\State $\mathbf{H}=[(\Delta(e_{1}|\mathbf{S}_{0}),e_{1}),(\Delta(e_{2}|\mathbf{S}_{0}),e_{2}),\cdots,(\Delta(e_{\omega}|\mathbf{S}_{0}),e_{\omega})].$
    \State\textbf{MaxHeapify}$(\mathbf{H})$. 
	\While{$\mathbf{True}$:}
	\State $(\_\_,e^{*})=$heappop($\mathbf{H}$).
    \State$\mathcal{S}=\mathcal{S}\cup e^{*}$
    \If{$|\mathcal{S}|\geqslant K$}
    \State \textbf{break}
    \EndIf
    \State $\mathbf{A}^{-1}=\mathbf{A}^{-1}-\frac{\mathbf{A}^{-1}\bm{x}_{e^{*}}\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}}{1+\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}\bm{x}_{e^{*}}}$
	\State $(\_\_,e_{c})\leftarrow \mathbf{H}[1]$ .
	\While{$\mathbf{True}$:}
	\State \textbf{UPDATEMARGINAL} %$\Delta(e_{c}|\mathcal{S}_{k})\leftarrow \bm{x}_{e_{c}}^{T}\mathbf{A}^{-1}\bm{x}_{e_{c}}$
	%\State heapreplace$(\mathbf{H}, (\Delta(e_{c}|\mathcal{S}_{k}),e_{c}) )$
	%\State $(\_\_,opti)\leftarrow \mathbf{H}[1]$.
	
	\If{$opti==e_{c}$}
	\State \textbf{break}.
	\Else
	\State $e_{c}=opti$
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}








The Naive Greedy algorithm mainly utilize the Sherman-Morrison formular. As we know, the computation of a normal square matrix has a complexity no less than $d^{2}$. For example, the  Coppersmith–Winograd algorithm has a complexity of $O(d^{2.376})$. The Naive Lazy mainly utilize the matrix determinant lemma which can compute the determinant of the sum of an invertible matrix $\mathbf{A}$ and the dyadic product.
\paragraph{PREPROCESSING}
To facilitate the use of matrix determinant lemma, we should calculate the inverse of the matrix $\mathbf{A}=cI_{d}+\sum_{i\in \mathcal{A}}\bm{x}_{i}\bm{x}_{i}^{T}$

\paragraph{FINDMAX} As the determinant of matrix $\mathbf{A}$ is positive, the locally optimal choice at each stage for the D-optimal design satisfies:
\begin{align}
\begin{split}
e^{*}&=\underset{e\in \Omega\setminus\mathcal{S}}{\mathbf{argmax}}~~ f_{D}(\mathcal{S}\cup e)-f_{D}(\mathcal{S})\\&=\underset{e\in \Omega\setminus\mathcal{S}}{\mathbf{argmax}}~~\mathop{\log\det}(\mathbf{A}+\bm{x}_{e}\bm{x}_{e}^{T})-\mathop{\log\det}(\mathbf{A})\\&=
\underset{e\in \Omega\setminus\mathcal{S}}{\mathbf{argmax}}~~\mathop{\log}\mathop{\det}(1+\bm{x}_{e}^{T}\mathbf{A}^{-1}\bm{x}_{e})
\end{split}
\end{align}
where $\mathbf{A}=\mathcal{F}(\mathcal{A},\mathcal{S})\in \mathbb{S}_{+}^{d}$. We have the  result based on the matrix determinant lemma. As the logarithmic function is monotonic, the choice satisfies:
\begin{align}\label{eq:naive}
    e^{*}&=\underset{e\in \Omega\setminus\mathcal{S}}{\mathbf{argmax}}~~  d_{e}
\end{align}
where $d_{e}=\bm{x}_{e}\mathbf{A}^{-1}\bm{x}_{e}$.

\paragraph{UPDATES} For each iteration step, we add a new element $e^{*}$ to our objective set $\mathcal{S}$, we can see that for the objective function, if we still want to use Eq.~\eqref{eq:naive} to find the locally optimal solution of further iteration, we should also update the matrix inverse of  $\mathbf{A}$. We use the trick of Sherman-Morrison formula to further decrease the complexity of matrix inverse.
\begin{lemma}
(Sherman–Morrison formula) Suppose 
$\mathbf{A}\in
\mathbb{R}^{d\times d}$ is an invertible matrix and 
$\bm{x}\in\mathbb{R}^{d}$ are column vector. Then $\mathbf{A}+\bm{x}\bm{x}^{T}$ is invertible if 
$1+\bm{x}^{T}\mathbf{A}^{T}\bm{x}\neq 0$, then its inverse is given by:
\begin{align}\label{eq: sherman-morrison}
(\mathbf{A}+\bm{x}\bm{x}^{T})^{-1}=\mathbf{A}^{-1}-\frac{\mathbf{A}^{-1}\bm{x}\bm{x}^{T}\mathbf{A}^{-1}}{1+\bm{x}^{T}\mathbf{A}^{-1}\bm{x}}    
\end{align}
\end{lemma}
This trick will also be very useful in Scalar Greedy algorithm which involved in Sec. \ref{sec:Scalar}. For the Naive Greedy algorithm, we update the matrix $\mathbf{A}_{k}^{-1}$ as follow:
\begin{align}\label{eq:adapt}
\begin{split}
\mathbf{A}_{k+1}^{-1}&=(\mathbf{A}_{k}+\bm{x}_{e^{*}}\bm{x}_{e^{*}}^{T})^{-1}\\&=\mathbf{A}_{k}^{-1}-\frac{\mathbf{A}_{k}^{-1}\bm{x}_{e^{*}}\bm{x}_{e^{*}}^{T}\mathbf{A}_{k}^{-1}}{1+\bm{x}_{e^{*}}^{T}\mathbf{A}_{k}^{-1}\bm{x}_{e^{*}}}
\end{split}
\end{align}



\paragraph{SUMMARY}



Greedy Algorithm is a polynomial time algorithm in the so-called \emph{value-oracle} model, i.e., presuming access to an oracle evaluating objective $f_{D}$ for any argument $\mathcal{S}\subseteq \Omega$. Indeed, it requires $O(KN^2)$ accesses to such an oracle.  Thus, the amount of time taken and the number of elementary operations performed by the algorithm differ by a constant factor. We notice that if we traverse all candidates directly, the constant will be a heavy load for computer and will not be realistic for a large dataset. In this section we detailed discuss how to accelerate the greedy optimization for D-optimal design. For all the algorithms, the input is:
\begin{algorithm}[H]
\begin{algorithmic}
\State \textit{Input}  $ \bm{x}_{1},\bm{x}_{2},\cdots,\bm{x}_{N}\in\mathbb{R}^{d},\mathcal{A}\in \mathcal{N}, \Omega \subseteq \mathcal{C}=\{(i,j):  i,j\in \mathcal{N}, i<j\},|\Omega|=\omega$.
\end{algorithmic}
\end{algorithm}



\paragraph{PREPROCESSING} We should prepare the $d_{e}$  and as we have discussed in Subsec. \ref{subsec:naive} it
should equal to $\bm{x}_{e}\mathbf{A}^{-1}\bm{x}_{e}$. In this procedure, we do:
\begin{algorithm}[H]
\begin{algorithmic}[1]
\State Calculate the inverse $\mathbf{A}^{-1}$.
\State Calculate $\mathbf{U}$: decompose the matrix $\mathbf{A}^{-1}$ into $\mathbf{U}^{T}\mathbf{U}$ by Cholesky decomposition.
	
\State Calculate and save  $\bm{z}_{i}=\mathbf{U}\bm{x}_{i}$ for all $i\in \mathcal{N}$. 
\State Calculate and save $d_{e}=||\bm{z}_{e_{i}}-\bm{z}_{e_{j}}||_{2}^{2}$ for all $e\in \Omega\setminus\mathcal{S}$.
\end{algorithmic}
\end{algorithm}
\paragraph{FINDMAX} $e^{*}=\underset{e\in \Omega\setminus\mathcal{S}}{\mathbf{argmax}}~~ d_{e}$.
\paragraph{UPDATES} In this procedure, we not only add element $e^{*}$ to the objective set but also update the $d_{e}$ by the scalar difference.
\begin{algorithm}[H]
\label{alg:greedy}
\begin{algorithmic}[1]
\State $\mathcal{S}=\mathcal{S}\cup e^{*}$
\State Calculate $\bm{v}=\frac{\mathbf{A}^{-1}\bm{x}_{e^{*}}}{\sqrt{1+\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}\bm{x}_{e^{*}}}}$.
\State Calculate and save  $z_{i}=\bm{v}^{T}\bm{x}_{i}$ for all $i\in \mathcal{N}$.
\State $d_{e}=d_{e}-(z_{e_{i}}-z_{e_{j}})^{2}$ for all $e\in \Omega\setminus\mathcal{S}$.
\State $\mathbf{A}^{-1}=\mathbf{A}^{-1}-\bm{v}\bm{v}^{T}$.  
\end{algorithmic}
\end{algorithm}



Instead of calculating inner product between square matrix and vector, we can calculate the vector norm. 

The algorithm uses the same main greedy process, and the preprocessing procedure and update procedure are also same with the na\"ive algorithm. We only change the calculation of $d_{e}$.  First, we factorize the matrix $\mathbf{A}^{-1}$ into $\mathbf{U}^{T}\mathbf{U}$, calculate and save the  $z_{i}=\mathbf{U}\bm{x}_{i}$ for $i\in\mathcal{N}$. Then, we calculate 
$d_{e}=||\bm{z}_{e_{i}}-\bm{z}_{e_{j}}||_{2}^{2}$ for  $e\in \Omega\setminus\mathcal{S}$. The other process would be same with the na$\"i$ve greedy.



The complexity for matrix inverse and CL factorization is $O(d^{2})$. The complexity to compute   $\mathbf{U}\bm{x}_{i}$ for  $i\in {\mathcal{N}}$ is $O(Nd^{2})$. The complexity to compute   $||\mathbf{U}\bm{x}_{i}-\mathbf{U}\bm{x}_{j}||_{2}^{2}$ is $O(N^{2}d)$ 
We repeat the above procedure multiple times, the total complexity is $O(N^{2}dK+Nd^{2}K+d^{2}K)$. 



The complexity is  
At the beginning, we build up a dictionary $d_{e}$ for every $e \in \Omega$, the $d_{e}$ is same as the first iteration's $d_{e}=||\mathbf{U}\bm{x}_{i}-\mathbf{U}\bm{x}_{j}||_{2}^{2}$ in Factorization Greedy algorithm. The $d_{e}$ should be saved and be used for locally optimal value  selection for next iterations. To update the $d_{e}$, we first calculate the scalar value
$z_{i}=\bm{v}_{k}^{T}\bm{x}_{i}$ for all $i\in\mathcal{N}$. The difference between current iteration's  $d_{e}$ and previous iteration's $d_{e}$ is $-(z_{i}-z_{j})^{2}$. 
We propose the  Scalar Greedy algorithm which use the advantage of Naive Greedy and Factorization Greedy.

For batch size $K$ query, the total complexity is $O(d^{2}K+Nd^{2}+N^{2}K)$.






















\begin{algorithm}[H]
\caption{Lazy Greedy with Heap}\label{alg:heap}
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $\mathbf{A}_{0}, \bm{x}_{1},\bm{x}_{2},\cdots,\bm{x}_{N}\in\mathbb{R}^{d}, \mathcal{C}=\{(i,j):  i,j\in \mathcal{N}, i<j\}$
   
	\State $\mathbf{H}=[(\bm{x}_{i,j}\mathbf{A}_{0}^{-1}\bm{x}_{i,j},(i,j)) for ~~ all~~ (i,j)\in \mathcal{C}]$.
    \State $(\mathbf{H})$ for all the $d_{i,j}$.
    \State $k=0$.
	\While{$k< K$}
	\State $d_{i,j}=$heap.popMax()
	\State $r^{*}=(i,j)$.
    \State$\mathcal{S}=\mathcal{S}\cup r^{*}$
    \State $k=k+1$.
	\State done=$\mathbf{False}$
	\State $\mathbf{A}_{k}^{-1}=\mathbf{A}_{k-1}^{-1}-\frac{\mathbf{A}_{k-1}^{-1}\bm{x}_{r^{*}}\bm{x}_{r^{*}}^{T}\mathbf{A}_{k-1}^{-1}}{1+\bm{x}_{r^{*}}^{T}\mathbf{A}_{k-1}^{-1}\bm{x}_{r^{*}}}$
	\While{$\mathbf{not}$ done:}
	\State $d_{i,j}\leftarrow \bm{x}_{i,j}^{T}\mathbf{A}_{k}^{-1}\bm{x}_{i,j}$.
	\State $d_{i^{'},j^{'}}=$heap.popMax().
	\If{$d_{i,j}\geqslant d_{i^{'},j^{'}}:$}
	\State done=$\mathbf{True}$.
	\State heap.insert$(d_{i^{'},j^{'}})$.
	\Else
	\State heap.insert$(d_{i,j})$.
	\State $d_{i,j}=d_{i^{'},j^{'}}$
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Heap Lazy Greedy}\label{alg:heaplazy}
\begin{algorithmic}[1]
	\State\textit{Initialize
	$\mathcal{S}=\emptyset, f, \Omega$}
    %\State\textit{Input} $f, \Omega$,$|\Omega|=\omega$
	%\State Build up  tuples   $(\Delta(e|\mathcal{S}_{0})=f(e)-f(\emptyset), e)$ for all $e\in \Omega$.
	%\State $\mathbf{H}=[(\Delta(e_{1}|\mathbf{S}_{0}),e_{1}),(\Delta(e_{2}|\mathbf{S}_{0}),e_{2}),\cdots,(\Delta(e_{\omega}|\mathbf{S}_{0}),e_{\omega})].$
    %\State\textbf{MaxHeapify}$(\mathbf{H})$.
    \State $\textbf{PREPROCESSING}$
    \State $\textbf{MAXHEAP}(f,\Omega)$
	\While{$|\mathcal{S}|<K$}
	\State $\textbf{FINDMAX}(\mathbf{H})$ 
	\State $\textbf{UPDATES}(\mathcal{S},e^{*})$ %$(\_\_,e^{*})=$heappop($\mathbf{H}$).
    %\State$\mathcal{S}=\mathcal{S}\cup e^{*}$
	%\State $(\_\_,e_{c})\leftarrow \mathbf{H}[1]$ .
	\While{$\mathbf{True}$}
	\State $\textbf{UPDATEMARGINAL}(\mathbf{H},e_{c},f)$ %$\Delta(e_{c}|\mathcal{S}_{k})\leftarrow f(\mathcal{S}_{k}\cup e_{c})-f(\mathcal{S}_{k})$
	%\State heapreplace$(\mathbf{H}, (\Delta(e_{c}|\mathcal{S}_{k}),e_{c}) )$
	%\State $(\_\_,opti)\leftarrow \mathbf{H}[1]$.
	
	\If{$opti==e_{c}$}
	\State $\textbf{break}$.
	\Else
	\State $e_{c}=opti$
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\Procedure{MAXHEAP}{$f,\Omega$}
\State Build up  tuples   $h_{e}=(\Delta(e|\mathcal{S}_{0}), e)$ for all $e\in \Omega$.
\State Build up a list $\mathbf{H}=[h_{1},h_{2},\cdots,h_{\omega}].$
\State Build-Max-Heap$(\mathbf{H})$.   
\EndProcedure
\Procedure{FindMax}{$\mathbf{H}$}
\State $(d_{e^{*}},e^{*})\leftarrow\text{Heap-Extract-Max}(\mathbf{H})$ 
\State $(d_{e_{c}},e_{c})\leftarrow\mathbf{H}[1]$
\EndProcedure
\Procedure{UpdateS}{$\mathcal{S},e^{*}$}
\State $\mathcal{S}=\mathcal{S}\cup e^{*}$ 
\EndProcedure

\Procedure{UPDATEMARGINAL}{$\mathbf{H},e_{c},f$}
\State $h_{1}\leftarrow(\Delta(e_{c}|\mathcal{S}_{k}),e_{c})$
\State $\mathbf{H}[1]\leftarrow h_{1}$
\State Max-Heapify $(\mathbf{H},1)$
\State $(\_\_,opti)\leftarrow\mathbf{H}[1]$.
\EndProcedure
\end{algorithmic}
\end{algorithm} 

\begin{algorithm}[H]
\caption{Memoization Heap Method}\label{basic}
\begin{algorithmic}[1] 
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $\mathbf{A}_{0}, \bm{x}_{1},\bm{x}_{2},\cdots,\bm{x}_{N}\in\mathbb{R}^{d}, \mathcal{C}=\{(i,j):  i,j\in \mathcal{N}, i<j\}$
    \State Decompose $\mathbf{A}_{0}^{-1}=\mathbf{U}_{0}^{T}\mathbf{U}_{0}$
    \State Calculate and save $z_{i}=\mathbf{U}_{0}\bm{x}_{i}$ for all $i\in\mathcal{N}$.
	\State Build up a dictionary for all   $d_{i,j}=||z_{i}-z_{j}||_{2}^{2},(i,j)\in \mathcal{C}$.
    \State\textbf{BUILD-MAX-HEAP}$(\mathbf{H})$ for all the $d_{i,j}$.
    \State $k=0$.
	\While{$k< K$}
	\State $d_{i,j}=$heap.popMax()
	\State $r^{*}=(i,j)$.
    \State
    $\mathcal{S}=\mathcal{S}\cup r^{*}$ 
    \State $k=k+1$.
	\State done=$\mathbf{False}$
	\State $\mathbf{A}_{k}^{-1}=\mathbf{A}_{k-1}^{-1}-\frac{\mathbf{A}_{k-1}^{-1}\bm{x}_{r^{*}}\bm{x}_{r^{*}}^{T}\mathbf{A}_{k-1}^{-1}}{1+\bm{x}_{r^{*}}^{T}\mathbf{A}_{k-1}^{-1}\bm{x}_{r^{*}}}$.
    \State Calculate and save $\bm{v}_{k-1}$, the $\bm{v}_{k-1}$ is given by Eq.\eqref{eq:decom}.
    \State Save  $\rho_{k-1,i}=\bm{v}_{k-1}\bm{x}_{i}$ for all $i\in \mathcal{N}$.
    \While{$\mathbf{not}$ done:}
	\State $d_{i,j}\leftarrow d_{i,j}-\underset{t\leqslant l< k }{\sum}(\rho_{l,i}-\rho_{l.j})^{2}$, $t$ is the last time $d_{i,j}$ was renewed.
	\State $d_{i^{'},j^{'}}=$heap.popMax().
	\If{$d_{i,j}\geqslant d_{i^{'},j^{'}}:$}
	\State done=$\mathbf{True}$.
	\State heap.insert$(d_{i^{'},j^{'}})$.
	\Else
	\State heap.insert$(d_{i,j})$.
	\State $d_{i,j}=d_{i^{'},j^{'}}$
    \EndIf
    \EndWhile
	\EndWhile
	\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}





\begin{algorithm}[H]
\caption{Heap Method-Yuan}\label{heap}
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $\mathbf{A}_{0}, \bm{x}_{1},\bm{x}_{2},\cdots,\bm{x}_{N}\in\mathbb{R}^{d}, \mathcal{C}=\{(i,j):  i,j\in \mathcal{N}, i<j\}$
    \State Calculate $\mathbf{U}_{0}$: decompose the matrix$\mathbf{A}_{0}^{-1}$ into $\mathbf{U}_{0}^{T}\mathbf{U}_{0}$ by cholesky decomposition.
    \State Calculate and save $z_{i}=\mathbf{U}_{0}\bm{x}_{i}$ for all $i\in\mathcal{N}$.
	\State Build up a dictionary for all   $d_{i,j}=||z_{i}-z_{j}||_{2}^{2}, (i,j)\in \mathcal{C}$.
    \State\textbf{BUILD-MAX-HEAP}$(\mathbf{H})$ for all the $d_{i,j}$. At the same time we save the renewed time $d_{i,j}.renew=0$
    \State $k=0$.
	\While{$k< K$}
	\State $d_{i,j}=$HEAP-EXTRACT-MAX($\mathbf{H}$).
	\State $r^{*}=(i,j)$.
    \State$\mathcal{S}=\mathcal{S}\cup r^{*}$
    \State $k=k+1$.
	\State done=$\mathbf{False}$
	\State $\mathbf{A}_{k}^{-1}=\mathbf{A}_{k-1}^{-1}-\frac{\mathbf{A}_{k-1}^{-1}\bm{x}_{r^{*}}\bm{x}_{r^{*}}^{T}\mathbf{A}_{k-1}^{-1}}{1+\bm{x}_{r^{*}}^{T}\mathbf{A}_{k-1}^{-1}\bm{x}_{r^{*}}}$
	\While{$\mathbf{not}$ done:}
	\State $d_{i,j}\leftarrow \bm{x}_{i,j}^{T}\mathbf{A}_{k}^{-1}\bm{x}_{i,j}$
	\State $d_{i,j}.renew=k$
	\State $\mathbf{H}[1]=d_{i,j}$
    \State MAX-HEAPIFY($\mathbf{H},1)$
    \State $d_{i,j}=\mathbf{H}[1]$
	\If{$d_{i,j}.renew==k$}
	\State done=$\mathbf{True}$.
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}





\begin{algorithm}[H]
\caption{Heap Memoization-Yuan}\label{heap}
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $\mathbf{A}_{0}, \bm{x}_{1},\bm{x}_{2},\cdots,\bm{x}_{N}\in\mathbb{R}^{d}, \mathcal{C}=\{(i,j):  i,j\in \mathcal{N}, i<j\}$
    \State Calculate $\mathbf{U}_{0}$: decompose the matrix$\mathbf{A}_{0}^{-1}$ into $\mathbf{U}_{0}^{T}\mathbf{U}_{0}$ by cholesky decomposition.
    \State Calculate and save $z_{i}=\mathbf{U}_{0}\bm{x}_{i}$ for all $i\in\mathcal{N}$.
	\State Build up a dictionary for all   $d_{i,j}=||z_{i}-z_{j}||_{2}^{2}, (i,j)\in \mathcal{C}$.
    \State\textbf{BUILD-MAX-HEAP}$(\mathbf{H})$ for all the $d_{i,j}$. At the same time we save the renewed time $d_{i,j}.renew=0$
    \State $k=0$.
	\While{$k< K$}
	\State $d_{i,j}=$HEAP-EXTRACT-MAX($\mathbf{H}$).
    \State$\mathcal{S}=\mathcal{S}\cup r^{*}$
    \State $k=k+1$.
	\State done=$\mathbf{False}$
	\State $\mathbf{A}_{k}^{-1}=\mathbf{A}_{k-1}^{-1}-\frac{\mathbf{A}_{k-1}^{-1}\bm{x}_{r^{*}}\bm{x}_{r^{*}}^{T}\mathbf{A}_{k-1}^{-1}}{1+\bm{x}_{r^{*}}^{T}\mathbf{A}_{k-1}^{-1}\bm{x}_{r^{*}}}$
	\State Calculate and save $\bm{v}_{k-1}$, the $\bm{v}_{k-1}$ is given by Eq.\eqref{eq:decom}.
    \State Save  $\rho_{k-1,i}=\bm{v}_{k-1}\bm{x}_{i}$ for all $i\in \mathcal{N}$.
	\While{$\mathbf{not}$ done:}
	\State $d_{i,j}\leftarrow d_{i,j}-\underset{t\leqslant l< k }{\sum}(\rho_{l,i}-\rho_{l.j})^{2}$, $t=d_{i,j}.renew$ is the last time $d_{i,j}$ was renewed.
	\State $d_{i,j}.renew=k$
	\State $\mathbf{H}[1]=d_{i,j}$
    \State MAX-HEAPIFY($\mathbf{H},1)$
    \State $d_{i,j}=\mathbf{H}[1]$
	\If{$d_{i,j}.renew==k$}
	\State done=$\mathbf{True}$.
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
\caption{LazyGreedy}\label{heap}
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $f, \Omega$,$|\Omega|=\omega$
	\State Build up  tuples for all   $(\Delta(e|\mathcal{S}_{0})=f(e)-f(\emptyset), e)$ for all $e\in \Omega$.
	\State $\mathbf{H}=[(\Delta(e_{1}|\mathbf{S}_{0}),e_{1}),(\Delta(e_{2}|\mathbf{S}_{0}),e_{2}),\cdots,(\Delta(e_{\omega}|\mathbf{S}_{0}),e_{\omega})].$
    \State\textbf{MaxHeapify}$(\mathbf{H})$. 
	\While{$\mathbf{True}$:}
	\State $(\_\_,e^{*})=$heappop($\mathbf{H}$).
    \State$\mathcal{S}=\mathcal{S}\cup e^{*}$
    \If{$|\mathcal{S}|\geqslant K$}
    \State \textbf{break}
    \EndIf
	\State $(\_\_,e_{c})\leftarrow \mathbf{H}[1]$ .
	\While{$\mathbf{True}$:}
	\State $\Delta(e_{c}|\mathcal{S}_{k})\leftarrow f(\mathcal{S}_{k}\cup e_{c})-f(\mathcal{S}_{k})$
	\State heapreplace$(\mathbf{H}, (\Delta(e_{c}|\mathcal{S}_{k}),e_{c}) )$
	\State $(\_\_,opti)\leftarrow \mathbf{H}[1]$.
	
	\If{$opti==e_{c}$}
	\State $\textbf{break}$.
	\Else
	\State $e_{c}=opti$
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
\caption{NaiveLazyGreedy}\label{heap}
\begin{algorithmic}[1]
	\State\textit{Initialize $\mathcal{S}=\emptyset$} 
    \State\textit{Input} $\mathbf{A}\in \mathbb{S}_{+}^{d}, \bm{x}_{1},\bm{x}_{2},\cdots,\bm{x}_{N}\in\mathbb{R}^{d}, \Omega=\{(i,j):  i,j\in \mathcal{N}, i<j\},|\Omega|=\omega$.
	\State Build up  tuples for all   $(\Delta(e|\mathcal{S}_{0})=\bm{x}_{e}^{T}\mathbf{A}^{-1}\bm{x}_{e}, e)$ for all $e\in \Omega$.
	\State $\mathbf{H}=[(\Delta(e_{1}|\mathbf{S}_{0}),e_{1}),(\Delta(e_{2}|\mathbf{S}_{0}),e_{2}),\cdots,(\Delta(e_{\omega}|\mathbf{S}_{0}),e_{\omega})].$
    \State\textbf{MaxHeapify}$(\mathbf{H})$. 
	\While{$\mathbf{True}$:}
	\State $(\_\_,e^{*})=$heappop($\mathbf{H}$).
    \State$\mathcal{S}=\mathcal{S}\cup e^{*}$
    \If{$|\mathcal{S}|\geqslant K$}
    \State \textbf{break}
    \EndIf
    \State $\mathbf{A}^{-1}=\mathbf{A}^{-1}-\frac{\mathbf{A}^{-1}\bm{x}_{e^{*}}\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}}{1+\bm{x}_{e^{*}}^{T}\mathbf{A}^{-1}\bm{x}_{e^{*}}}$
	\State $(\_\_,e_{c})\leftarrow \mathbf{H}[1]$ .
	\While{$\mathbf{True}$:}
	\State $\Delta(e_{c}|\mathcal{S}_{k})\leftarrow \bm{x}_{e_{c}}^{T}\mathbf{A}^{-1}\bm{x}_{e_{c}}$
	\State heapreplace$(\mathbf{H}, (\Delta(e_{c}|\mathcal{S}_{k}),e_{c}) )$
	\State $(\_\_,opti)\leftarrow \mathbf{H}[1]$.
	
	\If{$opti==e_{c}$}
	\State \textbf{break}.
	\Else
	\State $e_{c}=opti$
    \EndIf
\EndWhile
\EndWhile
\State\Return $\mathcal{S}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!t]
\begin{small}
\caption{Lazy Greedy Algorithm} \label{alg:lazygreedy}
Lazy Greedy Algorithm, as described in Sec.~\ref{sec:aclazy}. The main \textsc{Greedy} procedure, as well as \textsc{UpdateS}, are the same as in Alg.~\ref{alg:greedy}.
\begin{algorithmic}[1]
\Procedure {PreProcessing}{}
\State For all $e\in \Omega$, insert tuples $(\Delta(e|\emptyset),e)$ into heap $\mathbf{H}$.
\State Set $\mathcal{S} = \emptyset$.
\EndProcedure
\end{algorithmic}
\begin{algorithmic}[1]
\Procedure {FindMax}{$f,\mathcal{S}$}
\While{$\mathbf{True}$}
\State $(\Delta_{\texttt{old}},e)=$$\mathbf{H}$.\textsc{PopMax}()
\State Set $\Delta=\textsc{UpdateMarginal}(e,S)$
\State $(\Delta',e') = \mathbf{H}.$\textsc{Max}()
\If{$\Delta \geq \Delta'$}
\Return e
\Else
\State $\mathbf{H}$.\textsc{Insert}$\big( (\Delta,e )\big)$
\EndIf
\EndWhile 
\EndProcedure
\end{algorithmic}
\begin{algorithmic}[1]
\Procedure{UpdateMarginal}{$e,S$}
\State \Return $\Delta(e|\mathcal{ S})$
\EndProcedure
\end{algorithmic}
\end{small}
\end{algorithm}


\subsection{Fundamental Manipulation in Heap}.
\subsubsection{MAX-HEAPIFY}
In order to maintain the max-heap property, we call the procedure MAX-HEAPIFY. Its inputs are an array $\mathbf{H}$ and an index $i$ into the array. When it is called, MAX- HEAPIFY assumes that the binary trees rooted at LEFT.$i$ and RIGHT.$i$ are max- heaps, but that $\mathbf{H}[i]$  might be smaller than its children, thus violating the max-heap property. MAX-HEAPIFY lets the value at $\mathbf{H}[i]$ “float down” in the max-heap so that the subtree rooted at index $i$ obeys the max-heap property.
\begin{algorithm}[H]
\caption{MAX-HEAPIFY ($\mathbf{H},i$)}\label{heap}
\begin{algorithmic}[1]
\State $l$=LEFT.($i$)
\State $r$=RIGHT.($i$)	\If{$l\leqslant  \mathbf{H}$.heap\_size and $\mathbf{H}[l]> \mathbf{H}[i]$ }
\State $largest= l$
\Else
\State 
$largest= i$
\EndIf
\If{$r\leqslant \mathbf{H}$.heap\_size and $\mathbf{H}[r]> H[largest]$}
\State $largest=r$
\EndIf
\If{$largest\neq i$}
\State exchange $\mathbf{H}[i]$ with $\mathbf{H}[largest]$
\State MAX-HEAPIFY($\mathbf{H},largest$)
\EndIf
\end{algorithmic}
\end{algorithm}


\subsubsection{BUILD-MAX-HEAP}
\hspace{10pt}
\begin{algorithm}[H]
\caption{BUILD- MAX-HEAP($\mathbf{H}$)}\label{heap}
\begin{algorithmic}[1]
\For{$i=\left \lfloor  \mathbf{H}.length/2\right \rfloor \mathbf{downto} ~~1$}
\State MAX-HEAPIFY($\mathbf{H},i$)
\EndFor
\end{algorithmic}
\end{algorithm}

\subsubsection{HEAP-MAXIMUM}
Return $\mathbf{H}[1]$
\subsubsection{HEAP-EXTRACT-MAX}
\hspace{10pt}
\begin{algorithm}[H]
\caption{HEAP-EXTRACT-MAX ($\mathbf{H}$)}\label{heap}
\begin{algorithmic}[1]
\If{$\mathbf{H}.$heap\-size$<1$}
\State $\mathbf{error}$
\EndIf
\State $max=\mathbf{H}[1]$
\State $\mathbf{H}[1]=\mathbf{H}[\mathbf{H.}heap\-size]$
\State $\mathbf{H}.heap\-size=\mathbf{H}.heap\-size -1$
\State MAX-HEAPIFY($\mathbf{H},1$)
\State \Return{$max$}
\end{algorithmic}
\end{algorithm}

\subsubsection{HEAP-INCREASE-KEY}
\hspace{10pt}
\begin{algorithm}[H]
\caption{HEAP-INCREASE-KEY ($\mathbf{H},i,key$)}\label{heap}
\begin{algorithmic}[1]
\If{$key<\mathbf{H}[i]$}
\State $\mathbf{error}$
\EndIf
\State $\mathbf{H}[i]=key$
\While{$i>1$ and $\mathbf{H}[PARENT(i)]<\mathbf{H}[i]$}
\State exchange $\mathbf{H}[i]$ with $\mathbf{H}[PARENT(i)]$
\State $i=PARENT(i)$
\EndWhile
\end{algorithmic}
\end{algorithm}

\subsubsection{MAX-HEAP-INSERT}
\hspace{10pt}
\begin{algorithm}[H]
\caption{MAX-HEAP-INSERT($\mathbf{H},key$)}\label{heap}
\begin{algorithmic}[1]

\State $\mathbf{H}.heap\-size=\mathbf{H}.heap\-size+1$
\State $\mathbf{H}[\mathbf{H}.heap\-size]=-\infty$
\State HEAP-INCREASE-KEY($\mathbf{H},\mathbf{H}.heap\-size,key$)
\end{algorithmic}
\end{algorithm}




\input{tex/attach.tex}
\begin{figure*}[!t]
\centering
%\subfigure{\includegraphics[width=0.32\columnwidth]{pic/aucplotrop.pdf}}\hspace{-0.0cm}
%\subfigure{\includegraphics[width=0.32\columnwidth]{pic/aucplotsushi.pdf}}\hspace{-0.0cm}
%\subfigure{\includegraphics[width=0.32\columnwidth]{pic/aucplotnet.pdf}}
\includegraphics[width=2.0\columnwidth, height=0.8\columnwidth]{pic/testsushi.pdf}
\caption{\textcolor{red}{Test set  AUC for Sushi dataset, when comparisons samples are selected via Covariance, Fisher, Entropy and Random and Mutual Information. The classifier is trained via MAP \eqref{eq4} on the training set. Especially, for the Covariance method we record the execution time for Naive Greedy, Factorization Lazy and Scalar Lazy Greedy Algorithm.}}
\label{fig:aucsushi}
\end{figure*}


\begin{figure*}[!t]
\centering
%\subfigure{\includegraphics[width=0.32\columnwidth]{pic/aucplotrop.pdf}}\hspace{-0.0cm}
%\subfigure{\includegraphics[width=0.32\columnwidth]{pic/aucplotsushi.pdf}}\hspace{-0.0cm}
%\subfigure{\includegraphics[width=0.32\columnwidth]{pic/aucplotnet.pdf}}
\includegraphics[width=2.0\columnwidth, height=0.8\columnwidth]{pic/testnet.pdf}
\caption{\textcolor{red}{Test set  AUC for Netflix dataset, when comparisons samples are selected via Covariance, Fisher, Entropy and Random and Mutual Information. The classifier is trained via MAP \eqref{eq4} on the training set. Especially, for the Covariance method we record the execution time for Naive Greedy, Factorization Lazy and Scalar Lazy Greedy Algorithm.}}
\label{fig:aucnet}
\end{figure*}

\begin{figure*}[!t]
\centering
%\subfigure{\includegraphics[width=0.32\columnwidth]{pic/aucplotrop.pdf}}\hspace{-0.0cm}
%\subfigure{\includegraphics[width=0.32\columnwidth]{pic/aucplotsushi.pdf}}\hspace{-0.0cm}
%\subfigure{\includegraphics[width=0.32\columnwidth]{pic/aucplotnet.pdf}}
\includegraphics[width=2.0\columnwidth, height=0.8\columnwidth]{pic/testcamra2.pdf}
\caption{\textcolor{red}{Test set  AUC for Netflix dataset, when comparisons samples are selected via Covariance, Fisher, Entropy and Random and Mutual Information. The classifier is trained via MAP \eqref{eq4} on the training set. Especially, for the Covariance method we record the execution time for Naive Greedy, Factorization Lazy and Scalar Lazy Greedy Algorithm.}}
\label{fig:auccam}
\end{figure*}

